Evidence that PUBO outperforms QUBO when solving continuous optimization problems with the QAOA

Quantum computing provides powerful algorithmic tools that have been shown to outperform established classical solvers in specific optimization tasks. A core step in solving optimization problems with known quantum algorithms such as the Quantum Approximate Optimization Algorithm (QAOA) is the problem formulation. While quantum optimization has historically centered around Quadratic Unconstrained Optimization (QUBO) problems, recent studies show, that many combinatorial problems such as the TSP can be solved more efficiently in their native Polynomial Unconstrained Optimization (PUBO) forms. As many optimization problems in practice also contain continuous variables, our contribution investigates the performance of the QAOA in solving continuous optimization problems when using PUBO and QUBO formulations. Our extensive evaluation on suitable benchmark functions, shows that PUBO formulations generally yield better results, while requiring less qubits. As the multi-qubit interactions needed for the PUBO variant have to be decomposed using the hardware gates available, i.e., currently single- and two-qubit gates, the circuit depth of the PUBO approach outscales its QUBO alternative roughly linearly in the order of the objective function. However, incorporating the planned addition of native multi-qubit gates such as the global Molmer-Sorenson gate, our experiments indicate that PUBO outperforms QUBO for higher order continuous optimization problems in general.

==> txt/concept-FS.tex <==
% How do we build the QAOA for our specific problems (cont. and polynomial)?

% \begin{itemize}
%     \item Bit encoding
%     \item Unitary gate implementation of PUBO cost Hamiltonians (also breefly explain how the GMS gate can be used for this)
%     \item Selecting the benchmark functions (specifically also the regarded input domains)
% \end{itemize}

We will now discuss how we approached building the QAOA circuit from a continuous polynomial (objective) function. We will break our discussion down into the following sections
\begin{outline}
    \1[\ref{conceptDisc}] Discretization of the continuous (Objective) function.
    \1[\ref{conceptPuboHamil}] Defining the PUBO Hamiltonian
    \1[\ref{conceptCostHamil}] Using the Unitary gate implementation of multi-qubit interactions to build the QAOA cost Hamiltonian
\end{outline}
\subsection{Discretization}\label{conceptDisc}
All computational numerics require discretization. For us, this means binary discretization due to the architecture of the QGM's two-state basic units of information (Qubits).\\ 

We begin by imposing boundaries on the input domain of our continuous objective function. This is done because wider boundaries translate directly into larger Qubit requirements. To see this better, we introduce the following discretization procedure on our input domain:

\subsubsection{Bit-string representation of input domain}\label{conceptDisc:subsub:bitstring} We want to map from our input domain to a bit-string where each bit represents a power of 2, using the result of \eqref{binProof1}, where n represents the number of bit-strings (eg. n = 3 $\mapsto{}$ '000'). In order to reach decimal-place resolution, we will define bit-resolution as the number of negative powers we take 2 to. For example, bit-resolution 1 $\mapsto{} 2^{-1}$ and bit-resolution 2 $\mapsto{} (2^{-1}+2^{-2})$. The result of \eqref{binProof2} justifies this usage.
\begin{align*}
    \sum_{i=0}^{n}{2^i} & =2^{n+1}-1 \numberthis\label{binProof1}\\
    \lim_{k\rightarrow-\infty}\sum_{i=k}^{n}{2^i} & =2^{n+1} \numberthis\label{binProof2}
\end{align*}
Now, we need to map from an input domain $[a, b]\in\mathbb{R}$, to n in \eqref{binProof1}:
\\

For Input Domain $[a, b]\in\mathbb{R}$, $a<b$:
\begin{align*}
n: \mathbb{R}\times\mathbb{R} &\rightarrow \mathbb{Z}\\ \numberthis \label{domBitLen}
\{a,b\} &\mapsto{} {\lfloor{\ln_{2}{|max\{a,b\}|}}\rfloor} + 1
\end{align*}

And to keep track of negative domains, we define c as the negative domain flag:
\begin{align*}
c&\coloneqq\mathbb{I}_{\{a<0\}} \numberthis \label{negDomFlag}\\
\\\mathbb{I}_{\{a<0\}}&\coloneqq
 \begin{cases}
      1 & \text{if $a<0$}\\
      0 & \text{otherwise} 
    \end{cases}
\end{align*}
It should be noted that even though we have now obtained n, we still need further bits to define the discretization resolution. This will be addressed later in \eqref{bitstringDom}.
\\We finally have all the ingredients to develop our bit-string:\\\\
Using the formalism
\begin{align*}
    \text{Alphabet}&  &\Sigma&=\{0,1\}\\
    \text{Kleene star}& &\Sigma^*&=\bigcup^\infty_{i=0}\Sigma^i\\\\
    \text{Norm}& &\text{$|$ . $|$  :  }\Sigma^* &\rightarrow\mathbb{N}
\end{align*}\\
for a bit-string of length k, we define the language:\\
\begin{align*}
    \{0,1\}^k \coloneqq \{x\in\{0,1\}^* : |x|=k\} \numberthis\label{bitStringLang}
\end{align*}\\
For example, $\{0,1\}^2$ = $\{00,01,10,11\}$.\\\\
As such, we define our mapping from input domain [a, b], for n \eqref{domBitLen}, c \eqref{negDomFlag}, and some bit-resolution $r\in\mathbb{N}_0$, to a bit-string $\mathbb{S}$ as:\\
\begin{align*}
\mathbb{S} &\in \{0,1\}^{n+c+r} \numberthis\label{bitstringDom}\\
\mathbb{S} &\coloneqq s_{0}s_{1}...s_{n}s_{n+1}...s_{n+r}\numberthis \label{bitstringDef}
\end{align*}\\
Where
\begin{outline}
    \1 the bit order is flipped for $s_{1}...s_{n}$,
    \1 $s_{n+1}...s_{n+r}$ represent bit-resolutions of $2^{-1},..., 2^{-r}$,
    \1 and
        \begin{align*}
            s_{0}=
            \begin{cases}
                \{0,1\} & \text{if c = 1 \eqref{negDomFlag}}\\
                \varnothing & \text{if c = 0 \eqref{negDomFlag}}
            \end{cases}
        \end{align*}
\end{outline}
Finally, to put this all together, given any input domain [a, b] and bit-resolution r we define:

\begin{align*}
    \Phi: \mathbb{R}\ni[a, b] &\rightarrow \{0,1\}^{n+c+r}\numberthis\label{discMap}\\
    x_{[a, b]}^{(r)} &\mapsto{} \mathbb{S}
\end{align*}
Examples: 

$[0, 3]\ni2\mapsto{}'01'$ where the bit order is flipped, and $[-3, 3]\ni2\mapsto{} '001'$, to be read as '0-01', where the zeroth bit is reserved for the negative flag. That is, $\Phi(x_{[-3,3]}=-2) \text{ = } '101'$.\\\\
Example of a two variable domain: 

Let $(x, y)\in[-3, 3]\times[-3, 3]$. Then $\Phi(x = 3,y = -2)$ = $'011101'$, to be read as '0-11', '1-01'; and for $(x, y)\in[0,3]\times[-3,3]$, $\Phi(x = 3, y = 2)$ = $'11001'$, to be read as '11', '0-01'.\\\\
Example of a one variable domain with a bit-resolution of 2:

Let $x\in[-3, 3]$ and r = 2. Then $\Phi(x = -2.5)$ = $'10110'$, to be read as '1-01.10', and $\Phi(x^{(2)}_{[-1,1]} = -1.75)$ = $'1111'$, to be read as '1-1.11' \\\\

\subsubsection{Discretizing the objective function}\label{conceptDisc:subsub:objFen}
Now that we have discretized our input domain, we can finally move on to our objective function. First, using the pre-image of \eqref{discMap}, $\Phi^{-1}$, we need to define the following mapping:\\

Given any function $f: \mathbb{R}^d \rightarrow \mathbb{R}$, input domains of $[a_1,b_1]\times[a_2,b_2]\times...\times[a_d,b_d]$, bit-resolution r, and the corresponding bit-string $\mathbb{S}\coloneqq\mathbb{S}_1\mathbb{S}_2...\mathbb{S}_d$, we define

\begin{align*}
    \mathbb{D}^{f}&(\mathbb{S}) \coloneqq\\ 
    f&(\Phi^{-1}(\mathbb{S}_1\tilde{\mathbb{S}}_2...\tilde{\mathbb{S}}_d),\Phi^{-1}(\tilde{\mathbb{S}}_1\mathbb{S}_2...\tilde{\mathbb{S}}_d),...,\Phi^{-1}(\tilde{\mathbb{S}}_1...\mathbb{S}_d))\numberthis\label{eq:multiDomainPreDiscMap} \\
    \text{where} &\\
    &\tilde{\mathbb{S}}_j \coloneqq \text{ '00...0'} \text{, where the bit-string of variable $j$ is set to 0.}
    % &\mathbb{D}^{f}_i(\mathbb{S}) \coloneqq f(\Phi^{-1}(\mathbb{S}_i)) \text{ where $\mathbb{S}_j$ = '00...0' } \forall j \neq i\numberthis\label{eq:multiDomainPreDiscMapAtI}
    %{\{0,1\}}^{n_{i}+c+r} \rightarrow \mathbb{R}, \\
     %%%%%%%
\end{align*}
Using \eqref{eq:multiDomainPreDiscMap}, we can map from a bit-string back to the corresponding function output in $\mathbb{R}.$

We will now follow a simple example:\\ 

Let 
\begin{align*}
    g: [-3,3]\times[-3,3] &\rightarrow \mathbb{R}\\
    (x,y) &\mapsto{} x+y
\end{align*}
For a bit-resolution of 0, from Section \ref{conceptDisc:subsub:bitstring} we know that our bit-string has the format '$x_{0}x_{1}x_{2}y_{0}y_{1}y_{2}$'.
Therefore, for example for $\mathbb{S}$ = '001101':
\begin{align*}
    \mathbb{S} =  \mathbb{S}_x\mathbb{S}_y &= \text{ '001101',}\\
    \mathbb{D}^{g}('001101') &= g(\Phi^{-1}(\mathbb{S}_x\tilde{\mathbb{S}}_y), \Phi^{-1}(\tilde{\mathbb{S}}_x\mathbb{S}_y))\\
    &= g(\Phi^{-1}('001000'),\Phi^{-1}('000101'))\\
    &= g(2,-2) = 2 - 2 = 0
    % (x=2,y=-2) &\mapsto '001101'\\
    % \mathbb{D}_{x}^{f}('001101')&+\mathbb{D}_{y}^{f}('001101')\\
    % \mathbb{D}^{f}('001101') = f(\Phi^{-1}('001'))
    % =\Phi^{-1}(x_{[-3,3]} = 2) &+ \Phi^{-1}(y_{[-3,3]} = -2)\\
    % =2-2 &=0
\end{align*}
We now have a continuous objective function discretized in an input domain. Note that this domain, or specifically n+c+r in \eqref{bitstringDom} for each of our objective function's input variable, determines the number of Qubits we would ultimately need. Hence why wider boundaries and more resolution translates into larger resource (Qubit) requirement.
\subsection{PUBO Hamiltonian}\label{conceptPuboHamil}
So far, we have been working in a binary basis. As the prime step in developing our PUBO Hamiltonian, we need to flesh out an implementation of $\mathbb{D}^{f}(\mathbb{S})$ in terms of the spin basis that is native to quantum resources. To this end, we begin with the following:\\

Given any function $f: \mathbb{R}^d \rightarrow \mathbb{R}$, input domains of $[a_1,b_1]\times[a_2,b_2]\times...\times[a_d,b_d]$, bit-resolution r, $\Phi$ from \eqref{discMap} gives us the corresponding bit-string $\mathbb{S}\coloneqq\mathbb{S}_1\mathbb{S}_2...\mathbb{S}_d$. For which we know that:\\
\begin{align*}
    \mathbb{S} = \bigcup_{i=1}^{d}{\mathbb{S}_i}\\
    \text{where } {\mathbb{S}_i} \in \mathcal{L}_i\\
    \text{for } \mathcal{L}_i \coloneqq \{0,1\}^{n_i+c_i+r}\\
    \text{where we can define } \mathbb{L} \coloneqq \bigcup_{i=1}^{d}{\mathcal{L}_i}\\
    \text{and thus } \mathbb{S} \in \mathbb{L}
\end{align*}

Now for each bit-string variable $\mathbb{S}_i\in\mathcal{L}_i$, we set the pre-image of our d-dimensional bitstring $\Phi^{-1}(\tilde{\mathbb{S}}_1...\mathbb{S}_i...\tilde{\mathbb{S}}_d) \coloneqq \mathbb{X}_{i}$ \eqref{eq:multiDomainPreDiscMap}, and define it as:
\begin{align*}
    \mathbb{X}_{i} &\coloneqq (-2s_0+1)\sum_{j=1}^{n_i+r_i}{(\Phi^{-1}(\tilde{\mathbb{S}}_{i}^{j}))s_j}\numberthis\label{preImageProjection}\\
    \text{for } \tilde{\mathbb{S}}_{i}^{j} \coloneqq \tilde{s}_0\tilde{s}_1\tilde{s}_2...s_i...\tilde{s}_{n_i+r_i} &\text{ where $s_i = 1$ and $\tilde{s}_k \coloneqq 0$ $\forall k\neq i\wedge k=0$}
\end{align*}

Now that we have $\mathbb{X}_{i}$, we can address the mapping we need between the spin and binary basis. As such we introduce:
\begin{align*}
    \mathcal{T} : \{0,1\} &\rightarrow \{0,1\} \\
    s_k &\mapsto \frac{(1-\hat{\sigma}^z_k)}{2}\numberthis\label{}\\
\end{align*}
Where we have used the Pauli-Z operator $\hat{\sigma}^z$ to define the identity $\hat{\sigma}^z_k = 1-2s_k$.
% \begin{align*}
%     \mathcal{T}^{-1} : \{-1,1\} &\rightarrow \{0,1\} \\
%     \hat{\sigma}^z_k &\mapsto \frac{(1-\hat{\sigma}^z_k)}{2} = s_k\numberthis\label{}\\
% \end{align*}

We define $\mathbb{Z}_i$ as:
\begin{align*}
    \mathbb{Z}_i \coloneqq \mathcal{T}(\mathbb{X}_i)\numberthis\label{}
\end{align*}
Which gives us a format where we can use the output of a Pauli-Z operator measurement to assess our inputs.


Now that we have $\mathbb{Z}_{i}$, we can proceed to expanding on $\mathbb{D}^{f}(\mathbb{S})$ in spin basis:

\begin{align*}
    \mathbb{D}^{f}_{\sigma}(\mathbb{S}) = f(\mathbb{Z}_{1},\mathbb{Z}_{2},...,\mathbb{Z}_{d})\numberthis\label{}
\end{align*}

At this point, however, we finally have the PUBO hamiltonian of our objective function:
\begin{align*}
    \hat{\mathcal{H}}_C = \mathbb{D}^{f}_{\sigma}(\mathbb{S})\numberthis\label{}
\end{align*}

We follow a simple example:

Let 
\begin{align*}
    g: [-3,3] &\rightarrow \mathbb{R}\\
    x &\mapsto{} x^3
\end{align*}

For a bit-resolution of 0, we have $\mathbb{S}$ = $s_0s_1s_2$. From \eqref{preImageProjection}, we get:
\begin{align*}
    \mathbb{X}_x&=(-2s_0+1)(\Phi^{-1}(\hat{\mathbb{S}}^1)s_1+\Phi^{-1}(\hat{\mathbb{S}}^2)s_2)\\
    &=(-2s_0+1)(\Phi^{-1}((\tilde{s}_0s_1\tilde{s}_2))s_1+\Phi^{-1}((\tilde{s}_0\tilde{s}_1s_2))s_2)\\
    &=(-2s_0+1)(2s_2+s_1)\\
    &=s_1+2s_2-2s_0s_1-4s_0s_2
\end{align*}
\begin{align*}
    \mathbb{Z}_x=&\mathcal{T}(\mathbb{X}_x)\\
    =&\frac{(1-\hat{\sigma}^z_1))}{2}+2\frac{(1-\hat{\sigma}^z_2))}{2}-\\
    & 2\frac{(1-\hat{\sigma}^z_0))}{2}\frac{(1-\hat{\sigma}^z_1))}{2}-4\frac{(1-\hat{\sigma}^z_0))}{2}\frac{(1-\hat{\sigma}^z_2))}{2}\\
    =& 1.5\hat{\sigma}^z_0 - 0.5\hat{\sigma}^z_0\hat{\sigma}^z_1 - \hat{\sigma}^z_0\hat{\sigma}^z_2
\end{align*}
Now that we have $\mathbb{Z}_x$, we define

\begin{align*}
    \mathbb{D}^{g}_{\sigma}(\mathbb{S}) &= f(\mathbb{Z}_x)\\
    &= (\mathbb{Z}_x)^3\\
    &= {(1.5\hat{\sigma}^z_0 - 0.5\hat{\sigma}^z_0\hat{\sigma}^z_1 - \hat{\sigma}^z_0\hat{\sigma}^z_2)}^3\\
    &= 9\hat{\sigma}^z_0 - 5\hat{\sigma}^z_0\hat{\sigma}^z_1 - 8.5\hat{\sigma}^z_0\hat{\sigma}^z_2 + 4.5\hat{\sigma}^z_0\hat{\sigma}^z_1\hat{\sigma}^z_2
\end{align*}
Where we have our PUBO Hamiltonian of g
\begin{align*}
    \hat{\mathcal{H}}_C &= \mathbb{D}^{g}_{\sigma}(\mathbb{S})\\
    &= 9\hat{\sigma}^z_0 - 5\hat{\sigma}^z_0\hat{\sigma}^z_1 - 8.5\hat{\sigma}^z_0\hat{\sigma}^z_2 + 4.5\hat{\sigma}^z_0\hat{\sigma}^z_1\hat{\sigma}^z_2
\end{align*}
The final circuit of this example can be found in Figure \ref{fig:puboCostHamilCircuit}, for $P = 1$, $\gamma$ = 0.05, $\beta$ = 0.25.
\subsection{From PUBO to QAOA cost Hamiltonian}\label{conceptCostHamil}
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{gfx/circuitOfExample.pdf}
    \caption{Circuit of worked out example in Section \ref{conceptPuboHamil}, for $P = 1$, $\gamma$ = 0.05, $\beta$ = 0.25.}
    \label{fig:puboCostHamilCircuit}
\end{figure*}
